Segmenter: Transformer for Semantic Segmentation

Image segmentation is often ambiguous at the level of individual image patches and requires contextual information to reach label consensus. In this paper we introduce Segmenter, a transformer model for semantic segmentation. In contrast to convolution-based methods, our approach allows to model global context already at the first layer and throughout the network. We build on the recent Vision Transformer (ViT) and extend it to semantic segmentation. To do so, we rely on the output embeddings corresponding to image patches and obtain class labels from these embeddings with a point-wise linear decoder or a mask transformer decoder. We leverage models pre-trained for image classification and show that we can fine-tune them on moderate sized datasets available for semantic segmentation. The linear decoder allows to obtain excellent results already, but the performance can be further improved by a mask transformer generating class masks. We conduct an extensive ablation study to show the impact of the different parameters, in particular the performance is better for large models and small patch sizes. Segmenter attains excellent results for semantic segmentation. It outperforms the state of the art on both ADE20K and Pascal Context datasets and is competitive on Cityscapes.

==> figures/decoder_cnn.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{svg/decoder_simple.pdf}
  \caption{Overview of the FA-CNN decoder.} 
  \label{fig:decoder_cnn}
\end{figure}


==> tables/_region_.tex <==
\message{ !name(models.tex)}
\message{ !name(models.tex) !offset(-2) }
\begin{table}
\small
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{llcccc}
  \toprule
  Method & Backbone & Patch size & Im/sec & ImNet acc. & mIoU (SS) \\
  % \midrule
  % DeepLab V3+ & ResNet50-D & - & - & 43.95 \\
  % DeepLab V3+ & ResNet101-D & - & - & \textbf{45.47} \\
  % DeepLab V3+ & XCeption-65 & - & - & 45.0 \\
  \midrule
  Seg-Ti/16 & ViT-Ti & 16 & 396 & 78.6 & 39.03 \\
  \midrule
  Seg-S/32 & ViT-S & 32 & 1032 & 80.5 & 40.64 \\
  Seg-S/16 & ViT-S & 16 & 196 & 83.7 & 45.37 \\
  \midrule
  Seg-B\tsdagger/16 & DeiT-B & 16 & 92 & 85.2 & 47.08 \\
  \midrule
  Seg-B/32 & ViT-B & 32 & 516 & 83.3 & 43.07 \\
  Seg-B/16 & ViT-B & 16 & 92 & 86.0 & 48.06 \\
  Seg-B/8 & ViT-B & 8 & 7 & 85.7 & 49.54 \\
  \midrule
  Seg-L/16 & ViT-L & 16 & 33 & 87.1 & 50.71 \\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\caption{Performance comparison of different Segmenter models with varying backbones and input
  patch sizes on ADE20K validation set.}
\label{table:models}
\vspace{-0.5cm}
\end{table}

% experiments
% small_deit: ade_linear_datarefac_v0/deit_small_distilled_p16_224_linear_sgd_polynomial_aux0.0_im512/log.txt
% base_deit: ade_regularization_v0/deit_base_distilled_p16_384_linear_dropout0.0_droppath0.1_im512/log.txt
% base_vit: ade_regularization_v0/vit_base_p16_384_linear_dropout0.0_droppath0.1_im512/log.txt
% large_vit: ade_linear_baseline_v0/vit_large_p16_384_linear_sgd_polynomial_lr1e-3_im512/log.txt

\message{ !name(models.tex) !offset(-42) }


==> tables/ablation_mask.tex <==
\begin{table}[h]
\small
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{cccccc}
  \toprule
  Decoder & Layers & Token dim & Upsampling & \# Params & mIoU \\
  \midrule
  Linear & 0 & - & - & 0.1M & 47.21 \\
  \midrule
  CNN & 2 & 256 & 4 & 1.4M & \textbf{47.51} \\
  FA-CNN & 2 & 256 & 4 & 1.6M & 47.07 \\
  % \midrule
  % Mask & 1 & 768 & 1 & 9M & \textbf{47.72} \\
  \midrule
  Mask & 1 & 768 & 2 & 9M & 47.64 \\
  Mask & 2 & 768 & 2 & 16M & \textbf{47.77} \\
  Mask & 3 & 768 & 2 & 23M & 47.58 \\
  \midrule
  Mask & 2 & 384 & 2 & 4.2M & \textbf{47.38} \\
\bottomrule
\end{tabular}
\caption{Ablation of the decoder on ADE20K validation set. \todo{Is this table updated?}}
\label{table:ablation_mask_transformer}
\vspace{-0.1cm}
\end{table}


==> tables/decoder.tex <==
\begin{table}
\small
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{llccc}
\toprule
Model & Decoder & mIoU\\
\midrule
Seg-B/32 & Linear & 43.12 \\
\rowcolor{LightCyan}Seg-B-Mask/32 & Mask Transformer & 44.23 \\
\midrule
Seg-B\tsdagger/16 & Linear & 47.07 \\
\rowcolor{LightCyan}Seg-B\tsdagger-Mask/16 & Mask Transformer & 48.70 \\
\midrule
Seg-L/16 & Linear & 50.40 \\
\rowcolor{LightCyan}Seg-L-Mask/16 & Mask Transformer & 51.30 \\
\bottomrule
\end{tabular}
\caption{Performance comparison of different decoders on ADE20K validation set.}
\label{table:decoder}
\vspace{-0.3cm}
\end{table}


==> tables/inference.tex <==
\begin{table}
\small
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{llcc}
  \toprule
Method & Inference strategy & mIoU\\
\midrule
Seg-B & Token interpolation & 46.34 \\
Seg-B & Sliding window & 47.21 \\
Seg-B & Sliding window w/o averaging & 46.86 \\
\bottomrule
\end{tabular}
\caption{Comparison of different inference strategies.}
\label{table:inference}
\vspace{-0.1cm}
\end{table}


==> tables/sota_ade20k_test.tex <==
\begin{table}
\small
\setlength\tabcolsep{2.7pt} 
\centering
\begin{tabular}{llc}
\toprule
Method & Backbone & mIoU \\
\midrule
DRANet \cite{fu20} & ResNet-101 & 56.72 \\
\midrule
Ours & ? & ? \\
\bottomrule
\end{tabular}
\caption{State-of-the-art comparison on the ADE20K test dataset.}
\label{table:sota}
\end{table}


==> tables/sota_cityscapes_test.tex <==
\begin{table}
\small
\setlength\tabcolsep{2.7pt} 
\centering
\begin{tabular}{llcc}
\toprule
Method & Backbone & coarse & mIoU \\
\midrule
PSPNet \cite{zhao17} & ResNet-101 & \cmark & 80.2 \\
PSANet \cite{zhao18} & ResNet-101 & \cmark & 81.4 \\
DeepLabV3+ \cite{deeplabv3plus18} & Xception-71 & \cmark & 82.1 \\ 
DNL \cite{yin20} & HRNetV2-W48 & \cmark & 83.0 \\
OCR \cite{yuan20} & HRNetV2-W48 & \cmark & 84.2 \\
PSPNet \cite{zhao17} & ResNet-101 & \xmark & 78.4 \\
PSANet \cite{zhao18} & ResNet-101 & \xmark & 80.1 \\
DRANet \cite{fu20} & ResNet-101 & \xmark & 82.9 \\
OCR \cite{yuan20} & HRNetV2-W48 & \xmark & 83.6  \\
\midrule
Ours &  & \xmark & 79.55\\
\bottomrule
\end{tabular}
\caption{State-of-the-art comparison on the Cityscapes test dataset.}
\label{table:cityscapes_test}
\end{table}

